DKWS: A Distributed System for Keyword Search on Massive Graphs (Complete Version)

Due to the unstructuredness and the lack of schemas of graphs, such as knowledge graphs, social networks, and RDF graphs, keyword search for querying such graphs has been proposed. As graphs have become voluminous, large-scale distributed processing has attracted much interest from the database research community. While there have been several distributed systems, distributed querying techniques for keyword search are still limited. This paper proposes a novel distributed keyword search system called $\DKWS$. First, we \revise{present} a {\em monotonic} property with keyword search algorithms that guarantees correct parallelization. Second, we present a keyword search algorithm as monotonic backward and forward search phases. Moreover, we propose new tight bounds for pruning nodes being searched. Third, we propose a {\em notify-push} paradigm and $\PINE$ {\em programming model} of $\DKWS$. The notify-push paradigm allows {\em asynchronously} exchanging the upper bounds of matches across the workers and the coordinator in $\DKWS$. The $\PINE$ programming model naturally fits keyword search algorithms, as they have distinguished phases, to allow {\em preemptive} searches to mitigate staleness in a distributed system. Finally, we investigate the performance and effectiveness of $\DKWS$ through experiments using real-world datasets. We find that $\DKWS$ is up to two orders of magnitude faster than related techniques, and its communication costs are $7.6$ times smaller than those of other techniques.

==> exp-query-performance-all-backup.tex <==
\begin{figure*}[tp]
	%\vspace{-0.2cm}
		\begin{minipage}{\linewidth}
	
		\begin{tabular}{cc}
		% 1.1
		\begin{minipage}[t]{0.24\textwidth} 
		\includegraphics[width=\textwidth]{./figures/dkws-baseline-yago.eps}
		\subcaption{\footnotesize Vary $\#$ of query keywords (YAGO3)}
		\label{fig:dkws-baseline-yago}
		\end{minipage}
		% 1.2
		\begin{minipage}[t]{0.24\textwidth} 
		\includegraphics[width=\textwidth]{./figures/dkws-baseline-webuk.eps}
		\subcaption{\footnotesize Vary $\#$ of query keywords  (WebUK)}
		\label{fig:dkws-baseline-webuk}
		\end{minipage}
	
		% 1.3
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-baseline-dblp.eps}
			\subcaption{\footnotesize Vary $\#$ of query keywords (DBLP)}
			\label{fig:dkws-baseline-dblp}
			\end{minipage}
			% 1.4
			\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-baseline-dbpedia.eps}
			\subcaption{\footnotesize Vary $\#$ of query keywords  (DBpedia)}
			\label{fig:dkws-baseline-dbpedia}
			\end{minipage}
			
	
		\end{tabular}
		
			
		\begin{tabular}{cc}
		% 2.1
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-yago.eps}
			\subcaption{\footnotesize Vary $\#$ of the workers (YAGO3)}
			\label{fig:dkws-vary-workers-yago}
			\end{minipage}
			
		% 2.2
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-webuk.eps}
			\subcaption{\footnotesize Vary $\#$ of the workers (WebUK)}
			\label{fig:dkws-vary-workers-webuk}
			\end{minipage}
	 % 2.3
	 \begin{minipage}[t]{0.24\textwidth} 
		\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-dblp.eps}
		\subcaption{\footnotesize Vary $\#$ of the workers (DBLP)}
		\label{fig:dkws-vary-workers-dblp}
		\end{minipage}
	% 2.4
	\begin{minipage}[t]{0.24\textwidth} 
		\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-dbpedia.eps}
		\subcaption{\footnotesize Vary $\#$ of the workers (DBpedia)}
		\label{fig:dkws-vary-workers-dbpedia}
		\end{minipage}
	
	
		\end{tabular}



		\begin{tabular}{cc}
			% 3.1
			\begin{minipage}[t]{0.24\textwidth} 
				\includegraphics[width=\textwidth]{./figures/dkws-vary-tau-yago.eps}
				\subcaption{\footnotesize Vary $\#$ of $\tau$ (YAGO3)}
				\label{fig:dkws-vary-tau-yago}
				\end{minipage}
				
			% 3.2
			\begin{minipage}[t]{0.24\textwidth} 
				\includegraphics[width=\textwidth]{./figures/dkws-vary-tau-webuk.eps}
				\subcaption{\footnotesize Vary $\#$ of $\tau$ (WebUK)}
				\label{fig:dkws-vary-tau-webuk}
				\end{minipage}
		 % 3.3
		 \begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-vary-tau-dblp.eps}
			\subcaption{\footnotesize Vary $\#$ of $\tau$ (DBLP)}
			\label{fig:dkws-vary-tau-dblp}
			\end{minipage}
		% 3.4
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-vary-tau-dbpedia.eps}
			\subcaption{\footnotesize Vary $\#$ of $\tau$  (DBpedia)}
			\label{fig:dkws-vary-tau-dbpedia}
			\end{minipage}
		
		
			\end{tabular}


%%% top-k
			\begin{tabular}{cc}
				% 4.1
				\begin{minipage}[t]{0.24\textwidth} 
					\includegraphics[width=\textwidth]{./figures/dkws-vary-k-yago.eps}
					\subcaption{\footnotesize Vary $\#$ of top-$k$ (YAGO3)}
					\label{fig:dkws-vary-topk-yago}
					\end{minipage}
					
				% 4.2
				\begin{minipage}[t]{0.24\textwidth} 
					\includegraphics[width=\textwidth]{./figures/dkws-vary-k-webuk.eps}
					\subcaption{\footnotesize Vary $\#$ of top-$k$ (WebUK)}
					\label{fig:dkws-vary-topk-webuk}
					\end{minipage}
			 % 4.3
			 \begin{minipage}[t]{0.24\textwidth} 
				\includegraphics[width=\textwidth]{./figures/dkws-vary-k-dblp.eps}
				\subcaption{\footnotesize Vary $\#$ of top-$k$ (DBLP)}
				\label{fig:dkws-vary-topk-dblp}
				\end{minipage}
			% 4.4
			\begin{minipage}[t]{0.24\textwidth} 
				\includegraphics[width=\textwidth]{./figures/dkws-vary-k-dbpedia.eps}
				\subcaption{\footnotesize Vary $\#$ of top-$k$  (DBpedia)}
				\label{fig:dkws-vary-topk-dbpedia}
				\end{minipage}
			
			
				\end{tabular}


%%%%%%%% Followings are messages. For backup. 
\eat{
		\begin{tabular}{cc}
			% 3.1
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-baseline-msg-yago.eps}
			\subcaption{Vary $\#$ of query keywords (YAGO3)}
			\label{fig:dkws-baseline-msg-yago}
		\end{minipage}
		% 3.2
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-baseline-msg-webuk.eps}
			\subcaption{Vary $\#$ of query keywords (WebUK)}
			\label{fig:dkws-baseline-msg-webuk}
		\end{minipage}
		% 3.3
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-baseline-msg-dblp.eps}
			\subcaption{Vary $\#$ of query keywords (DBLP)}
			\label{fig:dkws-baseline-msg-dblp}
		\end{minipage}
			% 3.4
		\begin{minipage}[t]{0.24\textwidth} 
			\includegraphics[width=\textwidth]{./figures/dkws-baseline-msg-dbpedia.eps}
			\subcaption{Vary $\#$ of query keywords (DBpedia)}
			\label{fig:dkws-baseline-msg-dbpedia}
		\end{minipage}
		\end{tabular}
		
		\begin{tabular}{cc}
			% 4.1 
			\begin{minipage}[t]{0.24\textwidth} 
				\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-msg-yago.eps}
				\subcaption{\footnotesize Vary $\#$ of the workers (YAGO3)}
				\label{fig:dkws-vary-workers-msg-yago}
			\end{minipage}
				  % 4.2
			\begin{minipage}[t]{0.24\textwidth} 
				\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-msg-webuk.eps}
				\subcaption{\footnotesize Vary $\#$ of the workers (WebUK)}
				\label{fig:dkws-vary-workers-msg-webuk}
			\end{minipage}
				  % 4.3
				  \begin{minipage}[t]{0.24\textwidth} 
					\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-msg-dblp.eps}
					\subcaption{\footnotesize Vary $\#$ of the workers (DBLP)}
					\label{fig:dkws-vary-workers-msg-webuk}
				\end{minipage}
				% 4.4
				\begin{minipage}[t]{0.24\textwidth} 
					\includegraphics[width=\textwidth]{./figures/dkws-vary-workers-msg-dbpedia.eps}
					\subcaption{\footnotesize Vary $\#$ of the workers (DBpedia)}
					\label{fig:dkws-vary-workers-msg-dbpedia}
				\end{minipage}
		\end{tabular}
}		
	\caption{Performance of three keyword search semantics on the four datasets}
	\label{fig:performance}
		\end{minipage}
	%        \vspace{-1cm}
	\end{figure*}

==> msg.tex <==
\begin{table}[tb]
%\setlength{\abovecaptionskip}{10pt}
%\setlength{\belowcaptionskip}{10pt}
%\captionsetup{font={scriptsize}}
\caption{Messages (bytes) on YAGO3 (METIS, BFS, and Hash)}\label{table:yago-msg}
\vspace{-1ex}
\centering
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|}
  \hline
  {\bf Queries} & {\bf $|Q|$} & {\bf METIS} & {\bf BFS} & {\bf RANDOM} \\
  \hline
  $|Q_1|$ & 2 & 1,756,692 & 14,377,076 & 130,295,48  \\
  \hline
  $|Q_2|$ & 3 & 2,382,300 & 19,518,156 & 17,729,100 \\
  \hline
  $|Q_3|$ & 4 & 2,979,768 & 24,719,860 & 23,638,384 \\
  \hline
  $|Q_4|$ & 5 & 3,637,660 & 30,368,624 & 29,551,340 \\
  \hline
  $|Q_5|$ & 6 & 4,258,980 & 36,061,380 & 34,944,920 \\
  \hline
\end{tabular}
\end{scriptsize}
\end{table}


==> partition.tex <==
\begin{table}[tb]
%\setlength{\abovecaptionskip}{10pt}
%\setlength{\belowcaptionskip}{10pt}
%\captionsetup{font={scriptsize}}
\caption{Query time (rounds) on YAGO3 (METIS, BFS, and Hash)}\label{table:Statistics}
\vspace{-1ex}
\centering
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|}
  \hline
  {\bf Queries} & {\bf $|Q|$} & {\bf METIS} & {\bf BFS} & {\bf RANDOM} \\
  \hline
  $|Q_1|$ & 2 & 13.8786s (5) & 33.7877s (15) & 29.9985s (16) \\
  \hline
  $|Q_2|$ & 3 & 19.817s (5) & 50.7911s (20) & 43.1563s (16) \\
  \hline
  $|Q_3|$ & 4 & 26.4843s (5) & 61.058s (20) & 57.735s (16) \\
  \hline
  $|Q_4|$ & 5 & 30.8602s (5) & 80.7319s (20) & 72.1279s (16) \\
  \hline
  $|Q_5|$ & 6 & 40.3602s (5) & 93.0384s (20) & 85.9088s (16) \\
  \hline
\end{tabular}
\end{scriptsize}
\end{table}


==> symbolsofans.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tb!]
	\begin{scriptsize}
		\begin{center}
			{\renewcommand{\arraystretch}{1.35}
			\begin{tabular}{|p{25pt}|p{180pt}|} \hline Notation & Meaning \\
				\hline
                                \hline
                $O_{q}$ & Search origin of query keyword $q$\\ \hline
				$V_{q}$ & Vertices expanded by query keyword $q$ during $\bkws$\\ \hline
				$\VU$ & Vertices expanded by \textbf{\red{any}} of the query keywords during $\bkws$ \\ \hline
				$\VI$ & The root vertices of complete matches -- vertices expanded by \textbf{\red{all}} of the query keywords during $\bkws$\\ \hline
				$\VM$ & The root vertices of partial matches -- vertices expanded by \textbf{\red{not all}} of the query keywords during $\bkws$\\ \hline
			\end{tabular}}
		\end{center}
		\caption{Important vertex sets for the discussion of $\mathsf{bkws}$ and $\mathsf{fkws}$}
	  \label{tab-notations-ans}
	\end{scriptsize}
\end{table}


==> timecomm.tex <==
\begin{table}[tb]
%\setlength{\abovecaptionskip}{10pt}
%\setlength{\belowcaptionskip}{10pt}
%\captionsetup{font={scriptsize}}
\caption{Communication time on YAGO3 (METIS, BFS, and Hash)}\label{table:time-comm}
\vspace{-1ex}
\centering
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|}
  \hline
  {\bf Queries} & {\bf $|Q|$} & {\bf METIS} & {\bf BFS} & {\bf RANDOM} \\
  \hline
  $|Q_1|$ & 2 & 0.341036s & 1.0635s & 1.41622s  \\
  \hline
  $|Q_2|$ & 3 & 0.378606s & 1.50052s & 1.5557s \\
  \hline
  $|Q_3|$ & 4 & 0.343928s & 1.7609s & 1.29402s \\
  \hline
  $|Q_4|$ & 5 & 0.417992s & 1.83118s & 1.37774s \\
  \hline
  $|Q_5|$ & 6 & 0.364676s & 2.03432s & 1.66937s \\
  \hline
\end{tabular}
\end{scriptsize}
\end{table}


==> varypar.tex <==
\begin{table}[tb]
%\setlength{\abovecaptionskip}{10pt}
%\setlength{\belowcaptionskip}{10pt}
%\captionsetup{font={scriptsize}}
\caption{Vary partitions $|\F|$ on YAGO3}\label{table:partitions}
\centering
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|}
  \hline
  {\bf Queries} & {\bf $|Q|$} & {\bf 16-partitions} & {\bf 32-partitions} & {\bf 48-partitions} \\
  \hline
  $|Q_1|$ & 2 & 10.9626s & 10.7481s & 10.9888s  \\
  \hline
  $|Q_2|$ & 3 & 18.6174s & 14.434s & 15.0492s \\
  \hline
  $|Q_3|$ & 4 & 23.0062s & 19.5454s & 19.3826s \\
  \hline
  $|Q_4|$ & 5 & 28.7472s & 26.0689s & 23.1249s \\
  \hline
  $|Q_5|$ & 6 & 33.9236s & 30.5262s & 26.6821s \\
  \hline
\end{tabular}
\end{scriptsize}
\end{table}

